Boosting Feedback Efficiency of Interactive Reinforcement Learning by Adaptive Learning from Scores

Interactive reinforcement learning has shown promise in learning complex robotic tasks. However, the process can be human-intensive due to the requirement of a large amount of interactive feedback. This paper presents a new method that uses scores provided by humans instead of pairwise preferences to improve the feedback efficiency of interactive reinforcement learning. Our key insight is that scores can yield significantly more data than pairwise preferences. Specifically, we require a teacher to interactively score the full trajectories of an agent to train a behavioral policy in a sparse reward environment. To avoid unstable scores given by humans negatively impacting the training process, we propose an adaptive learning scheme. This enables the learning paradigm to be insensitive to imperfect or unreliable scores. We extensively evaluate our method for robotic locomotion and manipulation tasks. The results show that the proposed method can efficiently learn near-optimal policies by adaptive learning from scores while requiring less feedback compared to pairwise preference learning methods. The source codes are publicly available at https://github.com/SSKKai/Interactive-Scoring-IRL.

==> Sections/03_technical-approach-bk.tex <==

\section{Methodology} % Aim for a nice system figure at the beginning + a technical section with some math + a pseudocode algo 

In this section, we introduce our human-in-the-loop learning approach, which requires users to interactively score full trajectories of the learning agent to simultaneously learn the behavioral policy and reward function.
The reward function is trained as a neural network $\hat{r}_\theta$, users can choose either states or state-action pairs as the input. Our approach uses two replay buffers, one for the RL part to store the state-action transitions, and the other for the reward learning to store the trajectories and their scores. For policy learning, the only difference between our method and vanilla DRL algorithms is that the rewards are produced by the reward network, thus our approach can be applied to most off-policy DRL algorithms.
%As the reward learning part only affects the RL part by recalculating the reward values in the replay buffer after each reward update, our approach can fit with most off-policy DRL methods.

% XXX starts with a naive DRL agent generating a set of trajectories with poor performance, a human teacher then selects and scores some of these trajectories and the reward function is trained based on the rankings. The updated reward induces the RL agent to optimize the policy and generate trajectories with better performance. Training on the rankings of these better trajectories can then derive a more comprehensive and accurate reward function that enables the reinforcement agent to exceed its best performance again. By providing feedback intermittently during training in this way, we can continuously optimize the reward equation and thereby update the policy till optimal.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Learning to Reward from Global Scores}
%Given a set of trajectories $\tau_1, \tau_2,\ldots, \tau_m$ and their corresponding scores $l_1, l_2,\ldots,l_m$, we elicit the user's preference for any two trajectories by comparing their scores, and record them in a database $\mathcal{D}$ of triples ($\tau_i$, $\tau_j$, $\mu$) where $\mu$ is a preference label indicating which trajectory is more preferable for the user, e.g., $\mu=1$ if $l_i < l_j$. For $N$ trajectories, by scoring, we can obtain $N-1$ times more samples than directly giving the pairwise-preference feedback. We wish the parameterized reward function $\hat{r}_\theta$ can infer the underlying reward from scores and output the reward value that match user's evaluation standard, such that $\sum_{\tau_i}\hat{r}_\theta < \sum_{\tau_j}\hat{r}_\theta$ when $l_i < l_j$. To do so, we follow the basic learning-from-preference framework \cite{cao2007learning,christiano2017deep}. In this framework, by following the Bradley-Terry and Luce-Shephard models of preferences \cite{bradley1952rank,luce2012individual}, a preference predictor using the reward function $\hat{r}_\theta$ can be modeled as a softmax-normalized distribution as follow:

Given a set of trajectories $\tau_1, \tau_2,\ldots, \tau_m$ and their corresponding global scores $l_1, l_2,\ldots,l_m$, the user's preference over any pair of two trajectories is described by a distribution $\mu$, which can be derived by comparing their scores, e.g., $\mu=1$ if $l_i < l_j$. We parameterize a reward function $\hat{r}_\theta$ to infer the underlying reward from scores and output the reward value that matches the user's evaluation standard, such that $\sum_{\tau_i}\hat{r}_\theta < \sum_{\tau_j}\hat{r}_\theta$ when $l_i < l_j$. We follow the basic learning-from-preference framework \cite{cao2007learning,christiano2017deep} here. In this framework, by following the Bradley-Terry and Luce-Shephard models of preferences \cite{bradley1952rank,luce2012individual}, a preference predictor using the reward function $\hat{r}_\theta$ can be modeled as a softmax-normalized distribution as follows.

\begin{equation}\label{eq1}
    P(\tau_i \prec \tau_j) = \frac{exp\sum_{\tau_j}\hat{r}_\theta}{exp\sum_{\tau_i}\hat{r}_\theta + exp\sum_{\tau_j}\hat{r}_\theta}
\end{equation}

\noindent where $\tau_i \prec \tau_j$ denotes the trajectory $\tau_j$ is more preferred to the trajectory $\tau_j$. This equation demonstrates that the probability of preferring one trajectory to another is exponentially related to the predicted return of each trajectory. Thus, the parameterized reward function $\hat{r}_\theta$ can be learned via minimize the cross entropy loss between the predicted preference and the user's true preference as follows.

\begin{equation}\label{eq2}
    L(\theta) = -\sum_{(\tau_0, \tau_1, \mu) \in \mathcal{D}}[ \mu log P(\tau_i \prec \tau_j) + (1-\mu) log P(\tau_j \prec \tau_i) ]
\end{equation}

The preference distribution $\mu$ is usually a one-hot encoded label. Although this can learn reward effectively on correct labels, it may suffer from poor performance when there are wrong labels in the database $\mathcal{D}$. Unfortunately, it is nearly impossible for a human user to perfectly score a large number of trajectories. To strengthen the robustness against scoring error, we use the label smoothing method \cite{szegedy2016rethinking} to convert the hard label $\mu$ to soft label $\tilde{\mu}$ using $\tilde{\mu} = (1-\alpha)\mu + \alpha/K$, where $\alpha \in [0,1]$ is a constant factor that indicates the smoothing strength for one-hot label and $K$ denotes the number of labels, in our case, $K=2$. However, in our setting, using a constant smoothing strength for all pairwise labels may not be ideal because it ignores the relative relationship implicit in the score differences. It is intuitive that for a pair of trajectories with different scores, the larger the scores differ, the more confident that one trajectory is better than the other. Thus, to better exploit the information from human scores, we make the smoothing strength adaptive to the score differences by calculating the value of $\alpha$ as $\alpha = 1/(|l2-l1|+\alpha^\prime)^{2}$ where $\alpha^\prime$ is a hyperparameter. The adaptive $\alpha$ makes the label $\tilde{\mu}$ closer to 0 or 1 when pairwise trajectories significantly differ in the score and approach 0.5 when the scores are similar. Hence, the soft label $\tilde{\mu}$ is computed as:

\begin{equation}\label{eq3}
    \tilde{\mu} = (1-\frac{1}{(|l2-l1|+\alpha^\prime)^{2}})\mu + \frac{1}{K(|l2-l1|+\alpha^\prime)^{2}}
\end{equation}

Additionally, to further increase the robustness to vague and approximate scores, when the difference between the scores of two trajectories is less than a threshold $k$, we consider these two trajectories to be equally good and assign the label $\mu=0.5$ to both of them.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Data-Efficient Trajectory Sampling}
%As previously mentioned, there are two sampling processes in reward learning. One is to sample the newly generated trajectories for the human teacher to score. The other is to sample a batch of trajectory pairs from the scored trajectories for the reward update.
The reward learning process goes through two samplings. The first is to sample the newly generated trajectories of the RL agent for teachers to score. The other is to sample a batch of trajectory pairs from the scoring buffer that stores all scored trajectories.

\subsubsection{Sampling newly generated trajectories to score}
{\color{red}{Our approach periodically queries the user to score the newly generated trajectories of the RL agent and store these scored trajectories $(\tau, l)$ in the scoring buffer $\mathcal{D}$. Asking users to score all the trajectories can be burdensome, thus we aim to select the most informative scoring queries so that even if only a few newly generated trajectories are scored each time, they are still sufficient to train an appropriate reward. We use K-Means clustering to automatically sample the most differentiated trajectories in performance that are approximated by the predicted rewards. To sample K trajectories, we use the reward network to calculate the episodic return of each trajectory, then perform K-means clustering on these returns and find the trajectories whose returns are closest to each k centroid.}}
%In order to make our sampler pay more attention to newly generated trajectories instead of the scored trajectories, we propose a method to minimize the number of scored trajectories while maximizing the information entropy to ensure the data sufficiency.
%For sampling the newly generated trajectories to score, We want to reduce the number of the scored trajectories for the sample efficiency, while keeping them as diverse and informative as possible to ensure that these scoring trajectories are sufficient to train a comprehensive reward. Users can select the trajectories they believe have the greatest difference to score, but XXX also allows for automatic sampling. To sample K trajectories from the past experience, we use the reward network to calculate the return of each trajectory, then perform K-means clustering on these returns to find the trajectory that is closest to each centroid.

\subsubsection{Sampling scored trajectories to update reward}
%Given the scored trajectories, we wish the reward update can be faster and more accurate. Thus, in this work further we investigate methods for sampling from scoring buffer $\mathcal{D}$. Our intuition is that when a higher-scoring trajectory is sampled into $\mathcal{D}$, we should compare it more broadly with other trajectories, allowing the reward equation to learn what behaviors lead to higher scores. Inspired by the prioritized experience replay (PER) methods \cite{schaul2015prioritized} usually used in learning from demonstrations scheme, we make the trajectories with higher scores have a higher probability of being sampled. The sampling probability of each scored trajectory is calculated based on the corresponding score of each trajectory as follow:
For $n$ scored trajectories $(\tau, l)$ in scoring buffer $\mathcal{D}$, we can derive $(^{n}_{2})$ different trajectory pairs $(\tau_i, \tau_j, \tilde{\mu})$, but not all of them can lead to accurate reward update. Therefore, in this work, we further investigate methods for sampling from scoring buffer $\mathcal{D}$. Our intuition is that when a higher-scoring trajectory is sampled into $\mathcal{D}$, we should compare it more broadly with other trajectories, allowing the reward equation to learn what behaviors lead to higher scores. Inspired by the prioritized experience replay (PER) methods \cite{schaul2015prioritized} usually used in learning from demonstrations scheme, we propose the priority-based sampling scheme and make the trajectories with higher scores have a higher probability of being sampled. The sampling probability of each scored trajectory is calculated based on the corresponding score of each trajectory as follows.

\begin{equation}\label{eq4}
    P(i) = \frac{l_i^\beta}{\sum_k{l_k^\beta}}
\end{equation}

\noindent where $\beta$ is a hyperparameter that determines how much prioritization is assigned to a high-scored trajectory. And $k$ is the total number of trajectories in the scoring buffer.

We also investigate an additional sampling scheme employed by PEBBLE \cite{lee2021pebble}: entropy-based sampling, which randomly samples a large batch of trajectory pairs and seeks pairs that maximize the entropy $\mathcal{H}(P_\psi)$. We compare the effects of our method with uniform sampling and entropy-based sampling in experiments.

\begin{algorithm}[!ht]
\footnotesize
  \caption{Pseudo code of our algorithm}
  \label{alg:pseudocode}
  \renewcommand{\algorithmicforall}{\textbf{for each}}
  \begin{algorithmic}[1]
   \Require $J$, $K$, $M$, $N$, replay buffer $\mathcal{B}$, scoring buffer $\mathcal{D}$
    \Require Initialize policy $\pi_\psi$, critic $Q_\phi$, and reward $\hat{r}_\theta$
\Statex
    \Function{Main}{}
      \ForAll{episode}
      \State \Call{EnvironmentStep}{ }
      \If{episodes \% $K$ == 0}
        \State \Call{ScoreTrajectories}{$J$, $K$}
        \State \Call{UpdateReward}{$M$}
        \EndIf
      \State \Call{UpdatePolicy}{$N$}
    \EndFor
    \EndFunction
    
    \Statex
    \Function{EnvironmentStep}{ }
    \State Collect $\mathbf{s_{t+1}}$ by executing $\mathbf{a_t}=\pi_\psi(\mathbf{a_t}|\mathbf{s_t})$
    \State Generate reward from $r_t=\hat{r}_\theta(\mathbf{s_t})$ or $r_t=\hat{r}_\theta(\mathbf{s_t},\mathbf{a_t})$
    \State Store transitions $\mathcal{B}\leftarrow\mathcal{B}\cup{\{(\mathbf{s_t},\mathbf{a_t},r_t,\mathbf{s_{t+1}})\}}$
    \EndFunction
    
    \Statex
    \Function{ScoreTrajectories}{ }
    \State Sample $J$ trajectories $\tau_j$ from the latest $K$ in replay buffer $\mathcal{B}$
    \State Human teacher provides a score $l$ for each trajectory $\tau$
    \State Store $J$ scored trajectories $\mathcal{D}\leftarrow\mathcal{D}\cup{\{(\tau, l)\}}$
    \EndFunction
    
    \Statex
    \Function{UpdatePolicy}{ }
      \ForAll{policy gradient step}
      \State Sample $N$ transitions $(\mathbf{s_t},\mathbf{a_t},r_t,\mathbf{s_{t+1}})$ from $\mathcal{B}$
      \State Update $\pi_\psi$, $Q_\phi$ via policy gradient RL method, e.g., SAC
      \EndFor
    \EndFunction
    
    \Statex
    \Function{UpdateReward}{ }
      \ForAll{policy reward step}
      \State Sample $M$ pairwise scored trajectories $(\tau_i, \tau_j, l_i, l_j)$ from $\mathcal{D}$
      \State Make training batch $(\tau_i, \tau_j, \tilde{\mu})$ using eq.~\ref{eq3}
      \State Update $\hat{r}_\theta$ using eq.~\ref{eq2}
      \EndFor
      \State Relabel $\mathcal{B}$ by the updated $\hat{r}_\theta$
    \EndFunction

  \end{algorithmic}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Feedback-Efficient Policy and Reward Learning}
\label{sec:data_collection}
%XXX needs to leverage past experience as much as possible, as keeping teacher scores on a large number of trajectories can be both tedious and error-prone. We therefore adopt the off-policy learning methods. To enable the past experience available both for policy learning and reward learning, XXX assigns two buffers. One is the regular replay buffer $\mathcal{B}$ in the off-policy RL framework, storing all the past experience as transitions $(\mathbf{s_t},\mathbf{a_t},r_t,\mathbf{s_{t+1}})$ for learning policy. The user can either manually select or randomly sample some of the latest generated trajectories from the replay buffer $\mathcal{B}$ at intervals and score them based on their evaluation of the performance of the trajectories, then store these scored trajectories $(\tau, l)$ in a scoring buffer $\mathcal{D}$ for learning reward $\hat{r}_\theta$. Storing all scored trajectories in a scoring buffer enables the newly scored trajectories can also be used to compare with previously scored trajectories, which significantly improves the utilization of human feedback. 

%XXX needs to leverage past experience as much as possible, as keeping teacher scores on a large number of trajectories can be both tedious and error-prone. We therefore adopt the off-policy learning methods. To enable the past experience available both for policy learning and reward learning, XXX assigns two buffers. One is the regular replay buffer $\mathcal{B}$ in the off-policy RL framework, storing all the past experience as transitions $(\mathbf{s_t},\mathbf{a_t},r_t,\mathbf{s_{t+1}})$ for learning policy.

Algorithm \ref{alg:pseudocode} presents our method. It can be viewed as repeating two processes: the RL agent interacts with the environment and continuously generates new trajectories, and an off-policy DRL algorithm is applied to update the agent's policy $\pi_\psi$ to maximize the sum of the predicted reward generated by $\hat{r}_\theta$; While the teacher reviews the newly generated trajectories by video replay and scores them with a frequency $K$ during the RL training process, and store the scored trajectories $(\tau, l)$ in the scoring buffer $\mathcal{D}$ to update the reward network. The agent infers the teacher's preference from the score difference and optimizes the reward network accordingly. The updated reward network guides the agent to generate better-performing trajectories. Scoring these trajectories can lead to a more comprehensive reward network, and in this iterative process, the agent learns the optimal policy and reward simultaneously. Note that the reward function is dynamically updated during training, which may cause inconsistency in off-policy RL as the previously generated rewards cannot match the latest reward functions. Therefore we follow PEBBLE and relabel the replay buffer every time we update the reward.

Storing all scored trajectories in the scoring buffer enables the off-policy learning manner for reward learning. It allows newly scored trajectories to be compared with previously scored trajectories, significantly improving the utilization of human feedback. Additionally, the scoring buffer enables teachers to access the previous scores during training and correct them when they change their minds, which makes reward learning more robust.

{\color{red}{The scoring frequency $K$ and the number of trajectories to score each time $J$ can be unfixed and decided by the teacher according to the training process. In order to make the learning process more efficient, it is crucial to quickly derive a relatively accurate reward in the early stages of training. We use a faster scoring frequency at the beginning of training to get a sufficient number of scored trajectories and reward updates. To increase feedback efficiency, we slow down the scoring frequency when the agent's performance reaches a certain level. Although the quality of the collected trajectories may be poor at the beginning of training due to the naive policies, which may affect reward learning, in the trade-off between rewarding learning quality and speed, we found that such a frequency setting resulted in a more efficient learning process. Details in practical training can be referred to in the experiments section.}}

\begin{figure*}[!ht]
	\centering
    \subfigure[Mujoco Tasks]{%
    \includegraphics[height=5.5cm]{Graphics/figure2-1.pdf}%\hspace*{1em}
    \includegraphics[height=5.5cm]{Graphics/figure2-2.pdf}\label{2a}
    }%\hspace*{1em}
    \subfigure[Metaworld Tasks]{%
    \includegraphics[height=5.5cm]{Graphics/figure2-3.pdf}%\hspace*{1em}
    \includegraphics[height=5.5cm]{Graphics/figure2-4.pdf}\label{2b}
    }
    \caption{Learning curves of original SAC, PEBBLE and our approach on (a) locomotion tasks HalfCheetah and Ant in Mujoco simulation environment as measured on the ground true return; (b) robotic manipulation tasks ButtonPress and SweepInto in Metaworld simulation environment as measured on the success rate. The solid line and shaded regions represent the mean and min/max range across three runs, respectively.}
    \label{figure2} 
\end{figure*}

%Given the random behavior of a naive agent, the user gives these poorly performing trajectories a lower score at the beginning of training, such as 1.5 out of 10. The agent can then infer a reward function from these score differences, guiding the agent to generate trajectories that lead to higher human scores. Then, during the training, the updated behavior policy enables the reward function to extrapolate beyond its best performance by far, while the reward function guides the agent gradually towards the optimal policy that will get the highest score from the teacher as its continuous updating. In order to make the learning process more efficient, it is crucial to quickly derive a relatively accurate reward in the early stages of training. So the training process starts with a faster frequency of teacher scores, and to reduce the total number of scores, we slow down the frequency as the agent performs better.

%The reward value of each transition in the replay buffer is initially obtained from the reward network before it is stored. However, as the reward function is continuously updated based on human scores, the reward value labeled by the previous reward in the replay buffer can be inconsistent with the updated reward network, which can cause the learning process to be unstable. To address this issue, we relabel the entire replay buffer $\mathcal{B}$ every time the reward function is updated. Similarly, human teachers can access the scoring buffer $\mathcal{D}$ during the training process and correct their previous scores when they change their minds, making reward learning more stable. \textcolor{red}{Simplify the content which is the same with Pebble}

% \begin{algorithm}[!ht]
% \footnotesize
%   \caption{Pseudo code of our algorithm}
%   \label{alg:pseudocode}
%   \renewcommand{\algorithmicforall}{\textbf{for each}}
%   \begin{algorithmic}[1]
%    \Require $J$, $K$, $M$, $N$, replay buffer $\mathcal{B}$, scoring buffer $\mathcal{D}$
%     \Require Initialize policy $\pi_\psi$, critic $Q_\phi$, and reward $\hat{r}_\theta$
% \Statex
%     \Function{Main}{}
%       \ForAll{episode}
%       \State \Call{EnvironmentStep}{ }
%       \If{episodes \% $K$ == 0}
%         \State \Call{ScoreTrajectories}{$J$, $K$}
%         \State \Call{UpdateReward}{$M$}
%         \EndIf
%       \State \Call{UpdatePolicy}{$N$}
%     \EndFor
%     \EndFunction
    
%     \Statex
%     \Function{EnvironmentStep}{ }
%     \State Collect $\mathbf{s_{t+1}}$ by executing $\mathbf{a_t}=\pi_\psi(\mathbf{a_t}|\mathbf{s_t})$
%     \State Generate reward from $r_t=\hat{r}_\theta(\mathbf{s_t})$ or $r_t=\hat{r}_\theta(\mathbf{s_t},\mathbf{a_t})$
%     \State Store transitions $\mathcal{B}\leftarrow\mathcal{B}\cup{\{(\mathbf{s_t},\mathbf{a_t},r_t,\mathbf{s_{t+1}})\}}$
%     \EndFunction
    
%     \Statex
%     \Function{ScoreTrajectories}{ }
%     \State Sample $J$ trajectories $\tau_j$ from the latest $K$ in replay buffer $\mathcal{B}$
%     \State Human teacher provides a score $l$ for each trajectory $\tau$
%     \State Store $J$ scored trajectories $\mathcal{D}\leftarrow\mathcal{D}\cup{\{(\tau, l)\}}$
%     \EndFunction
    
%     \Statex
%     \Function{UpdatePolicy}{ }
%       \ForAll{policy gradient step}
%       \State Sample $N$ transitions $(\mathbf{s_t},\mathbf{a_t},r_t,\mathbf{s_{t+1}})$ from $\mathcal{B}$
%       \State Update $\pi_\psi$, $Q_\phi$ via policy gradient RL method, e.g., SAC
%       \EndFor
%     \EndFunction
    
%     \Statex
%     \Function{UpdateReward}{ }
%       \ForAll{policy reward step}
%       \State Sample $M$ pairwise scored trajectories $(\tau_i, \tau_j, l_i, l_j)$ from $\mathcal{D}$
%       \State Make training batch $(\tau_i, \tau_j, \tilde{\mu})$ using eq.~\ref{eq3}
%       \State Update $\hat{r}_\theta$ using eq.~\ref{eq2}
%       \EndFor
%       \State Relabel $\mathcal{B}$ by the updated $\hat{r}_\theta$
%     \EndFunction

%   \end{algorithmic}
% \end{algorithm}






